Representation Learning for cold-start recommendation

A standard approach to Collaborative Filtering (CF), i.e. prediction of user ratings on items, relies on Matrix Factorization techniques. Representations for both users and items are computed from the observed ratings and used for prediction. Unfortunatly, these transductive approaches cannot handle the case of new users arriving in the system, with no known rating, a problem known as user cold-start. A common approach in this context is to ask these incoming users for a few initialization ratings. This paper presents a model to tackle this twofold problem of (i) finding good questions to ask, (ii) building efficient representations from this small amount of information. The model can also be used in a more standard (warm) context. Our approach is evaluated on the classical CF problem and on the cold-start problem on four different datasets showing its ability to improve baseline performance in both cases.

==> added.tex <==
\section{Mixing Cold-start and Warm Recommendation}
\label{di}

We proposed two variants of IAM, one for the warm setting, and one other for the cold-start setting. An easy extension of our model can also allow one to smoothly move from cold-start to a \textit{warm} context : after having answer the interview, the user will start interacting with the system, and give new ratings, which can be integrated easily with our inductive translation model to update his representation. To do so, we simply change the learning paradigm of our model :
%We propose here an extension of this model allowing to smoothly move from cold-start to warm recommendation. The principle is to first ask questions to a new user (cold-start) and then to integrate the new incoming ratings made by this user among time without retraining the whole system. As far as we know this task is not usually studied in the recommender systems literature which focus on either warm systems or cold ones.\\
%The CSW-IAM model (Cold-start to Warm IAM) is learned in two steps:
\begin{itemize}
	\item First, the model is learned as in the warm setting described in Equation (8), i.e we learn each item's representation $q_i$ and the translations on representations (the $\Psi_i^r$ parameters).
	\item Secondly,  we select the most relevant items for the interview process by learning the $\alpha$'s weights using a $L_1$ regularization as explained in Equation (7). In this phase, we only learn the $\alpha$-values. %, the $z_i$ and $\Psi_i^r$ parameters have been learned in the previous step
%\begin{itemize}
%\item First, we learn the model in the warm setting as described in Equation (8). We thus learn for each item both its represntation $q_i$ and also how the user representations will be modified when a new rating will be provided (the $\Psi_i^r$ parameters). We thus obtain a good warm recommender system
%\item Second, we select the most relevant items to use at the beginning of the process by learning the $\alpha$'s weights using a $L_1$ regularization as explained in Equation (7). Note that, in this phase, we only learn the $\alpha$-values, the $z_i$ and $\Psi_i^r$ parameters have been learned in the previous step
\end{itemize}

The CSW-IAM is then used as followed: the non-null $\alpha$ are used for the initial interview, to compute an initial user representation following Equation (6). Then, each new incoming rating modifies the user representation as explained in Equation (4), resulting in a system that is naturally able to take into account new information. \\
This model has been evaluated on the Yahoo dataset with the following exprimental protocol: (i) the CSW-IAM is first evaluated in its cold-start setting, when the only ratings used are the ones selected by $\alpha$. Then, we evaluate the performance of this model by adding different amount of ''new'' ratings sampled uniformly from the set of items. The results are ilustrated in Figure XX and show that the performance of this model increases when new ratings are added, showing its ability to integrate this new information. We think that this CSW-Model is an interesting extension of IAM and CS-IAM , merging the cold-start and warm settings. 



==> additional.tex <==
\appendix

\newpage

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/jester_rmse"}
  \caption{RMSE}
  \label{fig:jester_RMSE}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/jester_accu"}
  \caption{Accuracy}
  \label{fig:jester_Accu}
\end{subfigure}
\caption{Dataset : \textbf{Jester} }
\label{fig:jester_alphadouble}
\end{figure}


\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/jester_30_rmse"}
  \caption{RMSE}
  \label{fig:jester_30_RMSE}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/jester_30_accu"}
  \caption{Accuracy}
  \label{fig:jester_30_Accu}
\end{subfigure}
\caption{Dataset : \textbf{Jester} }
\label{fig:jester_alphadouble}
\end{figure}



\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/yahoo_part_rmse"}
  \caption{RMSE}
  \label{fig:yahoo_RMSE}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/yahoo_part_accu"}
  \caption{Accuracy}
  \label{fig:yahoo_Accu}
\end{subfigure}
\caption{Dataset : \textbf{Yahoo} }
\label{fig:ml1M_alphadouble}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/yahoo_part_50_rmse"}
  \caption{RMSE}
  \label{fig:yahoo_50_RMSE}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/yahoo_part_50_accu"}
  \caption{Accuracy}
  \label{fig:yahoo_50_Accu}
\end{subfigure}
\caption{Dataset : \textbf{Yahoo} }
\label{fig:ml1M_alphadouble}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/ml1M_part_rmse"}
  \caption{RMSE}
  \label{fig:ml1M_RMSE}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/ml1M_part_accu"}
  \caption{Accuracy}
  \label{fig:ml1M_Accu}
\end{subfigure}
\caption{Dataset : \textbf{MovieLens 1M} }
\label{fig:ml1M_alphadouble}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/ml1M_part_100_rmse"}
  \caption{RMSE}
  \label{fig:ml1M_100_RMSE}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"Plot/ml1M_part_100_accu"}
  \caption{Accuracy}
  \label{fig:ml1M_100_Accu}
\end{subfigure}
\caption{Dataset : \textbf{MovieLens 1M} }
\label{fig:ml1M_alphadouble}
\end{figure}

\begin{table}
\begin{center}

\begin{tabular}{|l|l|c|} \hline 
Movie & Genre & $\alpha$ \\\hline
    Pleasantville (1998)& Comedy& 0.396737 \\
Mission: Impossible (1996)& Action|Adventure|Mystery& 0.384718 \\
Star Wars: Episode VI - Return of the Jedi (1983)& Action|Adventure|Romance|Sci-Fi|War& 0.252651\\
Patriot Games (1992)& Action|Thriller& 0.346994 \\
Lethal Weapon 3 (1992)& Action|Comedy|Crime|Drama& 0.413058  \\
Men in Black (1997)& Action|Adventure|Comedy|Sci-Fi& 0.412301 \\
Pulp Fiction (1994)& Crime|Drama& 0.317951 \\
Twelve Monkeys (1995)& Drama|Sci-Fi& 0.320635 \\
Crimson Tide (1995)& Drama|Thriller|War& 0.21444 \\
Mask, The (1994)& Comedy|Crime|Fantasy& 0.405714 \\
Back to the Future (1985)& Comedy|Sci-Fi& 0.351937 \\
Star Wars: Episode I - The Phantom Menace (1999)& Action|Adventure|Fantasy|Sci-Fi& 0.332822 \\
King Kong (1933)& Action|Adventure|Horror& 0.467331 \\
Who Framed Roger Rabbit? (1988)& Adventure|Animation|Film-Noir& 0.337147 \\
Rocky Horror Picture Show, The (1975)& Comedy|Horror|Musical|Sci-Fi& 0.428631 \\
Stargate (1994)& Action|Adventure|Sci-Fi& 0.308211 \\
Fantasia (1940)& Animation|Children's|Musical& 0.230316 \\
Time Bandits (1981)& Adventure|Fantasy|Sci-Fi& 0.341268 \\
Stand by Me (1986)& Adventure|Comedy|Drama& 0.393858 \\
Lost World: Jurassic Park, The (1997)& Action|Adventure|Sci-Fi|Thriller& 0.316492 \\
League of Their Own, A (1992)& Comedy|Drama& 0.347843 \\
Predator (1987)& Action|Sci-Fi|Thriller& 0.364581 \\
Jewel of the Nile, The (1985)& Action|Adventure|Comedy|Romance& 0.349509 \\
Say Anything... (1989)& Comedy|Drama|Romance& 0.425995 \\
West Side Story (1961)& Musical|Romance& 0.524218 \\
Broadcast News (1987)& Comedy|Drama|Romance& 0.472813 \\
Outbreak (1995)& Action|Drama|Thriller& 0.269675 \\ \hline
\end{tabular}
\end{center}
\caption{MovieLens 1M - An example of selected items for the interview process}
\label{tab:interview}
\end{table} 

 

==> exp_new.tex <==

\section{Experiments}
\label{exp}

\begin{table}[t]
\begin{subfigure}{.5\textwidth}
\begin{center}
\small{
\begin{tabular}{|c|c|c|c|} \hline 
DataSet & Users &  Items & Ratings  \\ \hline \hline
%
\textbf{ML1M} & 5,954 & 2,955 & 991,656 \\ \hline
%UserTrain & 2.962 & - & 490.627 \\ \hline
%UserTest  \textit{Answer set} & 2.992 & - & 250.466 \\\hline
%UTest \textit{Evaluation set} & - & - & 250.563 \\\hline \hline
%
\textbf{Flixter} & 35,657 & 10,247 &  7,499,706 \\\hline
%UserTrain & 17.802 & - & 3.702.429 \\\hline
%UserTest \textit{Answer set} & 17.855 & - & 1.899.181 \\\hline
%UTest \textit{Evaluation set} & - & - & 1.898.096 \\\hline \hline
%
\textbf{Jester} & 48,481 & 100 & 3,519,324  \\\hline
%UserTrain & 24.982 & - & 1.810.381 \\\hline
%UserTest \textit{Answer set} & 23.499 & - & 855.147 \\\hline
%UTest \textit{Evaluation set} & - & - & 853.796 \\\hline \hline
%
\textbf{Yahoo} & 15,397 & 1000 & 311,672 \\\hline
%UserTrain & 7.751 & - & 159.299 \\ \hline
%UserTest  \textit{Answer set} & 7.646 & - & 76.383 \\\hline
%UTest \textit{Evaluation set} & - & - & 75.990 \\\hline
\end{tabular}
}
\end{center}
\caption{Description of the datasets}
\label{tab:datasets}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
\begin{center}
\small{

\begin{tabular}{|c|c|c||c|} \hline 
     DataSet    & MF & IAM & ItemKNN \\\hline 
%
Jester  & 0.723       &  \textbf{0.737}   & 0.725 \\ %\hline
%
ML1M  &  0.689    &  \textbf{0.727} & 0.675 \\ %\hline
%
Yahoo   & 0.675   &  0.719         &  \textbf{0.726}\\ %\hline
%
Flixter   & \textbf{0.766}	  &  0.758   &  NA  \\ 
\hline
\end{tabular}

}
\end{center}
\caption{Accuracy of the different models in the classical CF context (without cold-start). NA (Not Available) means that, due to the complexity of ItemKNN, results were not computed over the Flixter dataset.}
\label{tab:IAM_accuracy}
\end{subfigure}
\caption{Datasets description and performance of different models.}
\vspace{-0.5cm}
\end{table}



\begin{figure}[t]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"yahoo_valid_rmse"}
  \caption{RMSE performance}
  \label{fig:yahoo_RMSE}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{"yahoo_valid_accuracy"}
  \caption{Accuracy performance}
  \label{fig:yahoo_Accu}
\end{subfigure}
\caption{Accuracy and RMSE evaluation on \textbf{Yahoo} dataset for all models, regarding the size of the interview (number of questions/items asked). }
\label{fig:yahoo_perf}
\end{figure}


We evaluate our models on four benchmark datasets - Table \ref{tab:datasets} - of various size in terms of number of users, of items or regarding the sparsity of ratings. The datasets are classical datasets used in the literature (\cite{zhou2011functional,golbandi2010bootstrapping}). \textbf{ML1M} corresponds to the \textit{MovieLens 1 millon} dataset and \textbf{Yahoo} corresponds to the \textit{Yahoo! Music} benchmark. \textbf{Flixter} and \textbf{Jester} are classical datasets. As our main goal is mainly to evaluate the quality of our approach in the context of \textit{new users} arriving in the system, we define the following protocol in order to simulate a realistic interview process on incoming users, and to evaluate different models. We proceed as follow: (i) We randomly divide each dataset along users, to have a pool of \textit{training} users denoted $\mathcal{U}^{train}$, composed of 50\% of the users of the complete dataset, on which we learn our model. The remaining users are split in two sets (representing each 25\% of initial users) for validation and testing. The interview process will be applied on each of these two subsets. (ii) The $\mathcal{U}^{test}$ and $\mathcal{U}^{valid}$  sets are then randomly split in two subsets of ratings to simulate the possible known answers : 50\% of the ratings of a set are used as the possible answers to the interview questions (\textit{Answer Set}). The 50\% of ratings left will be used for evaluating our models (\textit{Evaluation Set}).  Ratings have been binarized for each datasets, a rating of -1 (resp. 1) being considered a dislike, (resp. like).

\subsection{Models and Evaluation}
%
The quality of the different models is evaluated by two different measures. The \textit{root mean squared error} (RMSE) measures the average ratings' prediction precision measured as the difference between predicted and actual ratings $(\hat{r}_{u,i} - r_{u,i})^2$.  
% $ (\sum\limits_{u,i \in \mathcal{O}_{eval}} (\hat{r}_{u,i} - r_{u,i})^2)^{0.5} $. 
As we work with binary ratings, we also use the accuracy as a performance evaluation. In this context, it means that we focus on the overall prediction, i.e on the fact that the system has rightly predicted \textit{like} or \textit{dislike}, rather than on its precision regarding the "true" rating. The accuracy is calculated as the average "local" accuracy along users. These measures are computed over the set of missing ratings i.e the \textit{Evaluation Set}.  

 
%We define two types of accuracy : \textit{MacroAccuracy}, which is the mean of accuracy on all ratings, and \textit{MicroAccuracy}, which is the mean of each user's accuracy (?).
%The evaluation of our approach is made on two series of quantitative experiments. First, we will investigate the quality of our model in a \textit{warm-start} new user case, meaning that the system has access to all the potentially known ratings of the new users : to do so we use \textbf{IAM}, the Inductive-Additive Model defined by Equation \ref{eqiam_cf}. Second, we will explore the \textit{cold-start} user case with initialization interview process, using \textbf{CS-IAM}, the Cold-Start IAM, which optimizes Equation \ref{eqiam_cold}. 
%We present experiments on two of our models, firstly evaluating the ability of our approach to give prediction on a classic collaborative filtering case, then on a \textit{cold-start} situation. Therefore, we define :
%\begin{description}
%    \item[IAM], the Inductive-Additive Model which is presented in Equation \ref{eqiam_cf}
%    \item[CS-IAM], the Cold-Start IAM defined in Equation \ref{eqiam_cold}
%\end{description}

We explore the quality of our approach on both the classical CF context using the IAM Model (Equation \ref{eqiam_cf}) and on the cold-start problem using the CS-IAM model defined in Equation \ref{eqiam_cold}.  We compare our models with two baseline collaborative filtering methods: Matrix Factorization (MF) that we presented earlier, and the Item-KNN with Pearson correlation measure (\cite{koren2010factor}) which does not compute representations for users nor items but is a state-of-the-art CF method. Note that the inductive models (IAM and CS-IAM) are trained using only the set of training users $\mathcal{U}^{train}$. The ratings in the \textit{Answer Set} are only used as inputs during the testing phase, but not during training. Transductive models are trained using both the training users $\mathcal{U}^{train}$, but also the \textit{Answer set} of ratings defined over the testing users. % and thus use more information during training. 
It is a crucial difference as our model has significantly less information during training. % and therefore it is its true ability to generalize to new users (but with ''complete'' information) arriving in the system that is evaluated here. % XXRevoir model ItemKNN pearson pour voir argumentaire...XX

\begin{figure}[t]
\begin{subfigure}{0.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{"CSIAMPop_jest_valid"}
  \caption{Accuracy performance on \textbf{Jester}}
  \label{fig:jester_pop}
\end{subfigure}
\begin{subfigure}{0.6\textwidth}
  \centering
	\includegraphics[width=0.8\linewidth]{14visu}
  \caption{Visualization of some $\alpha_i \Psi_i$ after a PCA}
  \label{fig:2d}
\end{subfigure}
\caption{Performance on Jester, and visualization}
\vspace{-0.5cm}
\end{figure}


Each model has its own hyper-parameters to be tuned: the learning-rate of the gradient descent procedure, the size $N$ of the latent space, the different regularization coefficients... The evaluation is thus made as follows: models are evaluated for several hyper-parameters values using a grid-search procedure, the performance being averaged over 3 different randomly initialized runs. The models with the best average performance are presented in the next figures and tables. All models have been evaluated over the same datasets splits.


\subsection{Collaborative Filtering}
First, we evaluate the ability of our model to learn relevant representations in a classical CF context. In that case, the IAM model directly predicts ratings based on the ratings provided by a user. Results for the four different datasets are presented in Table \ref{tab:IAM_accuracy}. We can observe that, despite having much less information during the learning phase, IAM obtains competitive results, attesting the ability of the additive model to generalize to new users. More precisely, IAM is better than MF on three out of four datasets. For example, on the MovieLens-1M dataset, IAM obtains 72.8\% in terms of accuracy while MF's accuracy is only 70.8\%. Similar scores are observed for Jester and Yahoo. Although Item-KNN model gives slightly better results for two datasets, one should note that this method do not rely on nor provide any representations for users or items and belongs to a different family of approach. Moreover, ItemKNN - which is based on a KNN-based method - has a high complexity, and is thus very slow to use, and unable to deal with large scale datasets like Flixter on which many days are needed in order to compute performance.  Beyond its nice performance IAM is able to predict over a new user in a very short-time, on the contrary to MF and ItemKNN. 


% \begin{table}

% \caption{Comparison of accuracy on four different datasets XX accuracy / rmse / les deux ? accuracy lie au min average rmse ou max average accuracy -hyperparam different ? XX XX jamais itemKNN a temps pour flixter ?! XX }
% \begin{center}

% \begin{tabular}{|c|c|c|c|c||c|} \hline 
%      DataSet    & MeanRating & MatrixFacto  & IAM-S & IAM-D & ItemKNN \\\hline 
% %JEster RMSE     &   0.9528  & 0.8611      &  0.8422  & \textbf{0.8363}  & 0.8515 \\\hline
% Jester &   0.6308  & 0.7245      & 0.7354 &  \textbf{0.7388}   & 0.7249 \\ %\hline
% %
% %ML1M RMSE     & 0.9053  & 0.8766   & 0.8637  & 0.8606    & \textbf{0.8481}  \\\hline
% MovieLens 1M & 0.6829  & 0.7089    & 0.7291  & 0.7283  & \textbf{0.7311} \\ %\hline
% %
% %yahoo RMSE     &   0.9516   &  0.9434   &  0.9177  & 0.8856         &  \textbf{0.8394}\\\hline
% Yahoo &   0.6201   & 0.6728   &  0.7131  &  0.7183         &  \textbf{0.7433}\\ %\hline
% %
% %Flixter RMSE     &  0.9393    & 0.8116		      &   -    & 0.8414    &  -   \\\hline
% Flixter &  0.6532    & \textbf{0.7604}	 & 0.7491  &  0.7461   &  x  \\ 
% \hline
% \end{tabular}
% \end{center}
% \label{tab:IAM_accuracy}
% \end{table} 


\subsection{Cold-start Setting}



We now study the ability of our approach to predict ratings in a realistic cold-start situation. As MF and ItemKNN do not provide a way to select a set of items for the interview, we use two benchmark selection methods used in the literature (\cite{rashid2002getting}). The \textbf{POP} method select the most popular items - i.e the items with the highest number of ratings in the training set - and the \textbf{HELF} (\textit{Harmonic mean of Entropy and Logarithm of rating Frequency}) method which select items based on both their popularity but also using an entropy criterion, which focus on the \textit{informativeness} of items (e.g a controversial movie can be more informative than a movie liked by everyone) (\cite{rashid2008learning}). Here again, our model is learned solely on the $\mathcal{U}^{train}$  set. Baselines are computed on a dataset composed of the original $\mathcal{U}^{train}$  ratings with the additional ratings of the \textit{AnswerSet} of $\mathcal{U}^{test}$  that lie into the set of items selected by the POP or the HELF approach. Here again, transductive approaches use more information during training that our inductive model. 

The number of items selected by the CS-IAM model directly depends on the value of the $L_1$ regularization coefficient and several values have been evaluated.  In CS-IAM, the number of selected items correspond to the number of non-null $\alpha_i$ parameters. The number of items selected by POP and HELF is manually chosen.


Figure \ref{fig:yahoo_perf} shows accuracy and RMSE results for all models on the Yahoo dataset as a function of the interview size. It first illustrates that ItemKNN approach does not provide good results for RMSE-evaluation, as it is not a \textit{regression}-based method, but is better than MF in terms of accuracy. It also shows that HELF criterion does not seem to be specifically better on this dataset than the POP criterion. For both evaluations, CS-IAM gives better results, for all sizes of interview. It can also be noted that CS-IAM also gives good results when no item is selected due to the $\Psi_0$ parameters that correspond to the learned default representation. The model with $0$ items also expresses the base performance obtained on users unable to provide ratings during the interview. %\\ \hfill~ \linebreak

Detailed accuracy results for the four datasets are summarized in Table \ref{tab:BIAM_accuracy}, for different reasonable sizes of interview. Similar observations can be made on the results. While HELF criterion can improve the performance (for example on dataset Jester for both baselines models and on Flixter), CS-IAM managed to have the best accuracy for all datasets and all number of questions allowed.

%Figure \ref{fig:res} illustrates accuracy and RMSE results for all models at a given number of selected items. It first illustrates that the ItemKNN approach does not provide good results for RMSE-evaluation, as it is not a \textit{regression}-based method, but is better than MF in terms of accuracy. It also shows that HELF criterion does not perform better than POP XXsauf pour un dataset ??XX. For both evaluations, CS-IAM gives better results, for all sizes of interview.

 %For example, when selecting XX items on dataset XX, our approach obtain XX \% in term of accuracy while the baseline only obtain XX \% and XX\%. I

At last, when comparing the performance of CS-IAM with a version of IAM where items have been selected by the POP criterion -IAM-Pop, Figure \ref{fig:jester_pop} - one can see that the CS-IAM outperforms the other approaches. It interestingly shows that (i) IAM managed to give better results than MF with the same information selection strategy (POP) (ii) CS-IAM with all its parameters learned, managed to select more useful items for the interview process, illustrating that the performance of this model is due to both, its expressive power, but also on its ability to simultaneously learn representations, and select relevant items.

%We plot RMSE and accuracy regarding the number of questions asked (i.e, in our case, the number of non-negative $\alpha$ parameters).
%\\Figure ththt show that on the four datasets....
%\\





\begin{table}[t]
\begin{center}
\small{
\begin{tabular}{|c|c|c|c|c|c|c|}
	\cline{1-7}
	DataSet & NbItems & MF POP & MF HELF & IKNN POP & IKNN HELF & CS-IAM \\\hline\hline
    
	\multicolumn{1}{ |c  }{\multirow{4}{*}{Jester} } &
	
	\multicolumn{1}{ |c| }{5} & 0.603 & 0.589 & 0.608 & 0.634 & \textbf{ 0.667 } \\ %\cline{2-7}	
	\multicolumn{1}{ |c  }{}    &
	\multicolumn{1}{ |c| }{10} & 0.613 & 0.609 & 0.640 & 0.608 & \textbf{ 0.686 }  \\ %\cline{2-7}	
	\multicolumn{1}{ |c  }{}                        &
	\multicolumn{1}{ |c| }{20} & 0.665 & 0.641 & 0.688 & 0.676 &  \textbf{0.701 } \\ %\cline{2-7}
% 	\multicolumn{1}{ |c  }{}                        &
% 	\multicolumn{1}{ |c| }{30} & -     & -.667 & 0.698 & 0.696 &  0.722 (43)  \\ 
\hline\hline
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\multicolumn{1}{ |c  }{\multirow{4}{*}{MovieLens 1M} } &
	
	\multicolumn{1}{ |c| }{5} & 0.629 & 0.617 & 0.649 & 0.647 & \textbf{ 0.690  } \\ %\cline{2-7}	
	\multicolumn{1}{ |c  }{}  &
	\multicolumn{1}{ |c| }{10} & 0.634 & 0.620 & 0.651 & 0.653  &  \textbf{ 0.695 }  \\ %\cline{2-7}	
	\multicolumn{1}{ |c  }{}                        &
	\multicolumn{1}{ |c| }{20} & 0.648 & 0.621 & 0.663 & 0.638 &  \textbf{ 0.696  }  \\ %\cline{2-7}
% 	\multicolumn{1}{ |c  }{}                        &
% 	\multicolumn{1}{ |c| }{30} & 0.645 & - &  0.645 & - &   0.703 (36)\\ 
\hline\hline
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\multicolumn{1}{ |c  }{\multirow{4}{*}{Yahoo} } &
	
	\multicolumn{1}{ |c| }{5} & 0.590 & 0.594 & 0.623 & 0.624 &\textbf{ 0.638 }  \\ %\cline{2-7}	
	\multicolumn{1}{ |c  }{}  &
	\multicolumn{1}{ |c| }{10} & 0.601 & 0.610 & 0.633 & 0.634 & \textbf{ 0.647 } \\ %\cline{2-7}	
	\multicolumn{1}{ |c  }{}                        &
	\multicolumn{1}{ |c| }{20} & 0.621 & 0.623 & 0.654 & 0.654 &  \textbf{0.665}    \\ %\cline{2-7}
% 	\multicolumn{1}{ |c  }{}                        &
% 	\multicolumn{1}{ |c| }{30} & 0.658(40) & 0.657(40) & 0.685 & 0.692(40) &   0.690  \\  
\hline\hline
      
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{1}{ |c  }{\multirow{4}{*}{Flixter} } &
	
	\multicolumn{1}{ |c| }{5} & 0.719 & 0.722 & NA & NA & \textbf{0.723}   \\ %\cline{2-7}	
	\multicolumn{1}{ |c  }{}  &
	\multicolumn{1}{ |c| }{10} & 0.720 & 0.726 & NA & NA & \textbf{0.727}   \\ %\cline{2-7}	
	\multicolumn{1}{ |c  }{}                        &
	\multicolumn{1}{ |c| }{20} & 0.727 & \textbf{0.739} & NA  & NA & 0.735   \\ %\cline{2-7}
% 	\multicolumn{1}{ |c  }{}                        &
% 	\multicolumn{1}{ |c| }{30} & -     & - & x & x  & 0.703 (36)  \\ 
    
%     \cline{1-7}
\hline
\end{tabular}
}
\end{center}
\caption{Accuracy performance of models on four datasets regarding the number of questions asked. NA (Not Available) means that, due to the complexity of ItemKNN, results were not computed over the Flixter dataset.}
\label{tab:BIAM_accuracy}
\end{table} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Mixing Cold-start and Warm Recommendation}
%\label{di}

%We proposed two variants of IAM, one for the warm setting, and one other for the cold-start setting. An easy extension of 
Our model can also allow one to smoothly move from cold-start to a \textit{warm} context : after having answer the interview, the user will start interacting with the system, and give new ratings, which can be integrated easily with our inductive translation model to update his representation. To do so, we simply change the learning paradigm of our model :
%We propose here an extension of this model allowing to smoothly move from cold-start to warm recommendation. The principle is to first ask questions to a new user (cold-start) and then to integrate the new incoming ratings made by this user among time without retraining the whole system. As far as we know this task is not usually studied in the recommender systems literature which focus on either warm systems or cold ones.
%The CSW-IAM model (Cold-start to Warm IAM) is learned in two steps:
%\vskip -0.3cm
\begin{itemize}\itemsep0pt
	\item First, the model is learned as in the warm setting described in Equation (8), i.e we learn each item's representation $q_i$ and the translations on representations (the $\Psi_i^r$ parameters).
	\item Secondly,  we select the most relevant items for the interview process by learning the $\alpha$'s weights using a $L_1$ regularization as explained in Equation (7). In this phase, we only learn the $\alpha$-values. %, the $z_i$ and $\Psi_i^r$ parameters have been learned in the previous step
%\begin{itemize}
%\item First, we learn the model in the warm setting as described in Equation (8). We thus learn for each item both its represntation $q_i$ and also how the user representations will be modified when a new rating will be provided (the $\Psi_i^r$ parameters). We thus obtain a good warm recommender system
%\item Second, we select the most relevant items to use at the beginning of the process by learning the $\alpha$'s weights using a $L_1$ regularization as explained in Equation (7). Note that, in this phase, we only learn the $\alpha$-values, the $z_i$ and $\Psi_i^r$ parameters have been learned in the previous step
\end{itemize}
%\vskip -0.3cm
The CSW-IAM is then used as followed: the non-null $\alpha$ are used for the initial interview, to compute an initial user representation following Equation (6). Then, each new incoming rating modifies the user representation as explained in Equation (4), resulting in a system that is naturally able to take into account new information. \\
This model has been evaluated on the Yahoo dataset with the following exprimental protocol: (i) the CSW-IAM is first evaluated in its cold-start setting, when the only ratings used are the ones selected by $\alpha$. Then, we evaluate the performance of this model by adding different amount of ''new'' ratings sampled uniformly from the set of items. The results are ilustrated in Figure XX and show that the performance of this model increases when new ratings are added, showing its ability to integrate this new information. We think that this CSW-Model is an interesting extension of IAM and CS-IAM , merging the cold-start and warm settings. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
~\\
%\subsection{Qualitative Analysis}
We have shown that our approach gives significantly good quantitative results. We now focus our interest on a \textit{qualitative} analysis of the results performed over the MovieLens dataset. First, we compare the items selected by the three selection methods (CS-IAM, POP and HELF). These items are presented in Table \ref{tab:ml1M_interview}. First, when using the POP criterion, one can see that many redundant movies are selected - i.e the three last episodes of Star Wars on which the ratings are highly correlated: a user likes or  dislikes Star Wars, not only some episodes. The same effect seems to appear also with CS-IAM which selects \textit{Back to the future I} and \textit{Back to the future III}. But, in fact, the situation is different since the ratings on these two movies have less correlations. Half of the users that like \textit{Back to the future I} dislike \textit{Back to the future III}. At last, the lists provided by HELF and CS-IAM seem to be comparable from a qualitative point of view, but the list obtained by CS-IAM allows one to perform better in term of accuracy.

Figure \ref{fig:2d} shows the translations $\alpha_i\Psi_i$ after having performed a PCA in order to obtain 2D representations. What we can see is that depending on the movie, the fact of having a positive rating or a negative rating does not have the same consequences in term of representation:  For example, liking or disliking \textit{Saving Private Ryan} is different than liking or disliking \textit{Star Wars}; the translation concerning these two movies are almost perpendicular and thus result in a very different modification of the representation of the user. \textit{Schindler's List} has less consequences concerning the user representation i.e the norm of $\alpha_i \Psi_i^r$ is lower than the others. 
\begin{minipage}{\textwidth}
  \begin{minipage}[b]{0.35\textwidth}
	 \centering
       \includegraphics[width=\linewidth]{"sparsity_all"}
      \captionof{figure}{Accuracy along sparsity on \textbf{Yahoo}}
  \label{fig:sparsity_yahoo}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.65\textwidth}
    \centering
    
\small{
\begin{tabular}{|p{3cm}|p{3cm}|p{3cm}|} \hline 
\textbf{CS-IAM} & \textbf{Popularity} & \textbf{HELF}\\ \hline
American Beauty, Being John Malkovich, Lion King, Ghost, Superman, Back to the Future, Fargo, Armageddon, Get Shorty, Splash, 20 000 Leagues Under the Sea, Back to the Future Part III, Outbreak & 
American Beauty, Star Wars: Episode I,   Star Wars: Episode V, Star Wars: Episode IV, Star Wars: Episode VI, Jurassic Park,  Terminator 2,  Matrix,  Back to the Future,  Saving Private Ryan, Silence of the Lambs, Men in Black, Raiders of the Lost Ark, Fargo & 
Jurassic Park, Independence Day, Men in Black,  Total Recall, Mission: Impossible,  Speed, Face/Off,  Who Framed Roger Rabbit?, Abyss, Austin Powers, Beetlejuice,  Titanic \\ \hline
\end{tabular}
}
%\end{center}
\captionof{table}{MovieLens 1M - Selected items for the interview process by the three selection methods }
\vspace{-0.6cm}
\label{tab:ml1M_interview}

    \end{minipage}
  \end{minipage}


